Learning to Relate from Captions and Bounding Boxes

In this work, we propose a novel approach that predicts the relationships between various entities in an image in a weakly supervised manner by relying on image captions and object bounding box annotations as the sole source of supervision. Our proposed approach uses a top-down attention mechanism to align entities in captions to objects in the image, and then leverage the syntactic structure of the captions to align the relations. We use these alignments to train a relation classification network, thereby obtaining both grounded captions and dense relationships. We demonstrate the effectiveness of our model on the Visual Genome dataset by achieving a recall@50 of 15% and recall@100 of 25% on the relationships present in the image. We also show that the model successfully predicts relations that are not present in the corresponding captions.

==> 7-model.tex <==
\section{Proposed Model}
\label{model}

There are several alternate proposed models, as well as subtleties likely to be faced and a mathematical description of our losses, which we describe in the Appendix (Section \ref{appendix}). We also explain our detailed mathematical formulation in the Appendix.

\subsection{Motivation}
The primary motivation of our proposed architecture is to pool together information from various captions to construct a scene graph of the entire image. While a single caption captures only the central focus of an image, we hypothesize that across several images, different objects and the relations between them come into focus and are captioned. We thus aim to explore the formulation of a model that can construct more complete scene graphs than can be constructed by parsing a captioning pipeline (described in our baselines, Section \ref{baselines}).

\todo{Mask R-CNN; VGGNets and how well they generalize; Maxime's work on weak supervision; Gated Attention (distinction: we use a hard one-hot instead of sigmoid); Show, Attend and Tell}

\subsection{Model Overview and Proposed Architecture} \label{sec:modules}


In this architecture, we first propose using a FasterRCNN \citep{ren2015faster} to extract features from the image. These features then branch into: an entity branch, and a relation branch. The entity branch is a convolutional pipeline which ends in $e$ feature maps, where $e$ is a fixed constant representing the maximum number of entities the network can handle in its weakly constructed scene graph. Each feature map is accompanied by a classification vector of length $E+1$, where $E$ is the number of entity classes, the extra class being to represent a null entity. The objects present in the image and their classes can thus be represented by a $e\times(E+1)$ classification matrix $\mathbf{C_e}$. The relation branch is another convolutional pipeline that operates on all pairs of entity feature maps. Thus, the relation pipeline consists of $e*(e-1)$ feature maps, each representing a pair of entities. Each relation feature map has a corresponding classification vector of length $R+1$, where $R$ is the number of possible relations, and the extra dimension represents a \texttt{null} relation. The relations between the entities can thus be represented by a $e*(e-1)\times(R+1)$ classification matrix $\mathbf{C_r}$. Note that since we aim to construct a directed scene graph, the order in which the entities are considered is important. In each case, the classification vector is responsible for classifying the corresponding feature map into the correct entity and relation category respectively. 
 
\todo{Explain both train and test time}
\todo{In the future call this the 4 LSTM fork}
Our architecture has 4 LSTMs: a Selector LSTM, an Entity LSTM, a Relation LSTM, and a Connective LSTM. The Selector LSTM chooses between the Entity, Relation and Connective LSTMs as each word is generated. The Entity LSTM is responsible for producing a selection vector $\mathbf{s_e}$ of size $e$. This selection vector then selects one of the feature maps, and outputs the map's classification label as the caption word by doing $\mathbf{s_e}^T\times\mathbf{C_e}$. Similarly, the relation LSTM produces a selection vector $\mathbf{s_r}$ of size $e*(e-1)$ and outputs the relationship class as $\mathbf{s_r}^T\times\mathbf{C_r}$. In both these cases, the models should be forced to classify the feature maps correctly by using supervision from the corresponding caption word, since the caption word has to match the entity and relationship classification respectively. The Connective LSTM is chosen only when the Selector predicts that the next word (or set of words) in the caption is neither an entity nor a relation-- the Connective LSTM thus predicts words such as adjectives or stop-words. The entity and relation classification vectors can then be used to obtain a scene graph as follows: each entity classified as non-null forms a node in the scene graph, and non-null relations between two non-null entities form an edge in the scene graph.
